gamma-sky.net: Portal to the Gamma-Ray Sky

Gamma-sky.net is a novel interactive website designed for exploring the gamma-ray sky. The Map View portion of the site is powered by the Aladin Lite sky atlas, providing a scalable survey image tesselated onto a three-dimensional sphere. The map allows for interactive pan and zoom navigation as well as search queries by sky position or object name. The default image overlay shows the gamma-ray sky observed by the Fermi-LAT gamma-ray space telescope. Other survey images (e.g. Planck microwave images in low/high frequency bands, ROSAT X-ray image) are available for comparison with the gamma-ray data. Sources from major gamma-ray source catalogs of interest (Fermi-LAT 2FHL, 3FGL and a TeV source catalog) are overlaid over the sky map as markers. Clicking on a given source shows basic information in a popup, and detailed pages for every source are available via the Catalog View component of the website, including information such as source classification, spectrum and light-curve plots, and literature references. We intend for gamma-sky.net to be applicable for both professional astronomers as well as the general public. The website started in early June 2016 and is being developed as an open-source, open data project on GitHub (https://github.com/gammapy/gamma-sky). We plan to extend it to display more gamma-ray and multi-wavelength data. Feedback and contributions are very welcome!

==> Makefile <==
TARGET=gammaskynet-gamma2016
LATEX=pdflatex
BIBTEX=bibtex

all: $(TARGET).pdf

$(TARGET).pdf: *.tex figures/* text/* tables/* $(TARGET).bib

%.pdf: %.tex
	$(LATEX) $<
	$(BIBTEX) $*
	$(LATEX) $<
	$(LATEX) $<

make clean:
	- rm -f $(TARGET).pdf $(TARGET).aux $(TARGET).log $(TARGET).bbl $(TARGET).fff $(TARGET).tar.gz
	- rm -f *.aux */*.aux */*/*.aux

tarball:
	- tar -cvzf $(TARGET).tar.gz \
	$(TARGET).tex \
	$(TARGET).bib \
	$(TARGET).bbl \
	text/*.tex \
	tables/*.tex \
	figures/mapview_retake.PNG \
	figures/catview_retake.PNG \
	figures/four_images.png \
	figures/galactic_region_NEW.png \
	figures/cygnus_region.png \
	aip-cp.cls aipnum-cp.bst \
	Makefile

